"It's like a rubber duck that talks back": Understanding Generative AI-Assisted Data Analysis Workflows through a Participatory Prompting Study

Generative AI tools can help users with many tasks. One such task is data analysis, which is notoriously challenging for non-expert end-users due to its expertise requirements, and where AI holds much potential, such as finding relevant data sources, proposing analysis strategies, and writing analysis code. To understand how data analysis workflows can be assisted or impaired by generative AI, we conducted a study (n=15) using Bing Chat via participatory prompting. Participatory prompting is a recently developed methodology in which users and researchers reflect together on tasks through co-engagement with generative AI. In this paper we demonstrate the value of the participatory prompting method. We found that generative AI benefits the information foraging and sensemaking loops of data analysis in specific ways, but also introduces its own barriers and challenges, arising from the difficulties of query formulation, specifying context, and verifying results.

==> tables/tbl_part_old.tex <==
\begin{table*}
\caption{Participant profession and experience with spreadsheets (), programming (), and generative AI ()}
\label{tbl:demographics}
\begin{center}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{p{0.05\linewidth} p{0.20\linewidth} p{0.25\linewidth}
 p{0.25\linewidth} p{0.25\linewidth}}
P & 
Profession &
Spreadsheet\newline Experience & 
Programming\newline Experience &
Generative AI\newline Experience \\
\toprule
\toprule

1 & PhD candidate\newline (Anthropology) 
& A lot of experience,\newline but my use is basic 
& I have learnt a little bit,\newline but never used it 
& Heard of them,\newline but haven't tried any \\
\hline

2 & Consultant 
& A lot of experience,\newline but my use is basic 
& I have learnt a little bit,\newline but never used it 
& Occasionally use one or more \\
\hline

3 & Statistician 
& A lot of experience, and I use some advanced features 
& I have learnt a little bit,\newline but never used it 
& Occasionally use one or more \\
\hline

4 & Account Officer 
& A lot of experience,\newline but my use is basic 
& I have learnt a little bit, \newline but never used it 
& Heard of them,\newline but haven't tried any \\
\hline

5 & Student\newline (Geophysics) 
& A lot of experience, and I use some advanced features 
& I am moderately experienced, and write programs regularly 
& Regularly use one or more \\
\hline

6 & Software\newline Engineer 
& Some experience, but I'm still a beginner 
& I am moderately experienced and write programs regularly 
& Occasionally use one or more \\
\hline

7 & Data Analyst 
& A lot of experience, and I use some advanced features 
& I have learnt a little bit,\newline but never used it 
& Regularly use one or more \\
\hline

8 & Software\newline Engineer 
& A lot of experience, and I use some advanced features
& I am moderately experienced and write programs regularly 
& Regularly use one or more \\
\hline

9 & Student\newline (Informatics) 
& A lot of experience,\newline but my use is basic 
& I have learnt a little bit,\newline but never used it 
& Regularly use one or more \\
\hline

10 & PhD student\newline (History) 
& A lot of experience,\newline but my use is basic 
& I have learnt a little bit,\newline but never used it 
& Heard of them but haven't tried any \\
\hline

11 & PhD candidate\newline (Computer Science) 
& A lot of experience, and I use some advanced features 
& I am highly experienced 
& Regularly use one or more \\
\hline

12 & PhD student\newline (Anthropology) 
& A lot of experience,\newline but my use is basic 
& I know enough to use it for small infrequent tasks
& Occasionally use one or more \\
\hline

13 & Computer\newline Scientist 
& A lot of experience, and I use some advanced features 
& I am highly experienced 
& Casually tried one or more \\
\hline

14 & Student\newline (Philosophy)
& A lot of experience, and I use some advanced features 
& I know enough to use it for small infrequent tasks 
& Occasionally use one or more \\
\hline

15 & Student\newline (Nursing Science) 
& A lot of experience,\newline but my use is basic 
& I know enough to use it for small infrequent tasks 
& Occasionally use one or more \\

\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> tables/tbl_tasks.tex <==
\begin{table*}
\caption{Participant task description, initial prompt, and turns taken for that task}
\label{tbl:tasks}
\begin{center}
\renewcommand{\arraystretch}{1.4}

\begin{tabular}{p{0.01\linewidth} p{0.18\linewidth} p{0.66\linewidth} p{0.05\linewidth}}
{\small P} & 
{\small Description of task} &
{\small First prompt} & 
{\small Turns} \\
\midrule
{\scriptsize 1} 
& {\scriptsize Performing a literary analysis with spreadsheets}
& {\scriptsize I have a spreadsheet with data. In rows are the data for ``tales'' and in columns are the data for ``cooperative behaviour''. Each cell contains an example of a cooperative behaviour in a certain tale, e.g., ``brother saved brother''. I need a way to code each cell according to different categories. Explain how to use a spreadsheet for this with an example.}
& {\scriptsize 3} \\
{\scriptsize 2}
& {\scriptsize Categorizing age data in a spreadsheet}
& {\scriptsize I have data about people with a column for their age. I need to regroup the people with age between 18-35 into categories Gen X, Gen Y, Gen Z. Explain how to use a spreadsheet for this with an example.} 
& {\scriptsize 2} \\
{\scriptsize 3} 
& {\scriptsize Analysis on how discrimination impacts workplace performance} 
& {\scriptsize I am trying to determine the extent to discrimination affects employee performance in my company. What data is required? What online data sources may be relevant? Explain how to solve this in Excel with an example.}
& {\scriptsize 4} \\
{\scriptsize 4} 
& {\scriptsize Creating a reusable expense tracker in spreadsheet}
& {\scriptsize I am making a form in Excel where people have to categorize their business expenses. For each expense the user has to choose a category. Instead of typing out the category I want them to be able to filter on the cell. Explain how to do this in Excel with an example.}   
& {\scriptsize 4} \\
{\scriptsize 5} 
& {\scriptsize Data analysis exploration of ridesharing data} 
& {\scriptsize I have a dataset of rides taken on a bike sharing service. For each ride we know the rider type (casual or annual member), start and end points time and location, and bike type (classical or electric). I am trying to understand what differentiates the usage of the casual and annual members. Suggest a data analysis strategy for solving this problem using Excel and R.}
& {\scriptsize 4} \\
{\scriptsize 6} 
& {\scriptsize Apartment hunting organization} 
& {\scriptsize I am looking for an apartment. I have a spreadsheet with the data about various apartments and the following column headers: Name, Google Rating, Location, Distance from Msft, 2Br Price, \# of Baths, Sq. ft., Move-in Date, Notes. Explain a few ways I can analyse this data in a spreadsheet to help me make my decision.}  
& {\scriptsize 6} \\
{\scriptsize 7} 
& {\scriptsize Strategies to share data analyses}
& {\scriptsize I am a data analyst who does his analysis in Microsoft Excel. It is challenging to share the findings from my analysis because Excel files stored on my computer are not live, in the sense that I am the only one who can have access to it at any one point in time. Suggest a few solutions to this problem.} 
& {\scriptsize 3} \\
{\scriptsize 8} 
& {\scriptsize Writing Javascript code}
& {\scriptsize Write me javascript code that adds 2 days on top of current today and has these conditions: - When it's Monday/Tuesday/Wednesday/Thursday, then the day would be Wednesday/Thursday/Friday/Saturday - When it's Friday, then the day would be Monday - When it's Saturday/Sunday, the day would be Tuesday}  
& {\scriptsize 6} \\
{\scriptsize 9} 
& {\scriptsize Requesting analysis strategies for an HRI survey}
& {\scriptsize I am a researcher studying Human-Robot Interaction. I have data from a survey in which 100s of respondents were asked to rate their perception of two robot voices on a Likert scale from -3 to +3. I am interested in the differences between voices. Suggest a few analytical strategies for solving this problem. Suggest how to implement the strategies in Excel.}
& {\scriptsize 5} \\
{\scriptsize 10} 
& {\scriptsize Potential career paths based on background} 
& {\scriptsize I am a history PhD candidate with strong research, writing, and education skills. I would like to know what potential career paths I could follow based on my skills when I graduate.}
& {\scriptsize 7} \\
{\scriptsize 11} 
& {\scriptsize Comparing object detection models}
& {\scriptsize I'm interested in the performance of object detection models. Recommend ways to compare these models. Focus on accuracy, speed in ms, and size of the model.}   
& {\scriptsize 3} \\
{\scriptsize 12} 
& {\scriptsize Finding strategies for literary analysis}
& {\scriptsize I am interested in narrative structure. Recommend appropriate frameworks for analyzing narrative text within short stories. Cite your sources.}
& {\scriptsize 5} \\
{\scriptsize 13} 
& {\scriptsize Performing data analysis on student grading data} 
& {\scriptsize I want to disaggregate categorical and numerical grading data by gender as part of my research study. I want to calculate the difference between the median grade and each gender. How do I do this in a spreadsheet? After this is done, I would like to export the data to latex and create a visualization of the data, can you give me the steps to perform these tasks?}  
& {\scriptsize 5} \\
{\scriptsize 14} 
& {\scriptsize Discovering data about lifestyle impact on diabetic patients} 
& {\scriptsize Are type-2 diabetic patients compliant with lifestyle modifications? Cite your sources please.}
& {\scriptsize 3} \\
{\scriptsize 15} 
& {\scriptsize Understanding what factors impact working for corporations}
& {\scriptsize Does university curriculum prepare people for work in corporate organizations after graduation? I want to know the answer and all the potential factors that contribute to this. Please cite your references.}
& {\scriptsize 7} \\
\bottomrule
\end{tabular}
\end{center}
\end{table*}

